How to hide a clique?

In the well known planted clique problem, a clique (or alternatively, an independent set) of size $k$ is planted at random in an Erdos-Renyi random $G(n, p)$ graph, and the goal is to design an algorithm that finds the maximum clique (or independent set) in the resulting graph. We introduce a variation on this problem, where instead of planting the clique at random, the clique is planted by an adversary who attempts to make it difficult to find the maximum clique in the resulting graph. We show that for the standard setting of the parameters of the problem, namely, a clique of size $k = \sqrt{n}$ planted in a random $G(n, \frac{1}{2})$ graph, the known polynomial time algorithms can be extended (in a non-trivial way) to work also in the adversarial setting. In contrast, we show that for other natural settings of the parameters, such as planting an independent set of size $k=\frac{n}{2}$ in a $G(n, p)$ graph with $p = n^{-\frac{1}{2}}$, there is no polynomial time algorithm that finds an independent set of size $k$, unless NP has randomized polynomial time algorithms.

==> algorithm.tex <==
\section{Main algorithm}\label{sec:algorithm}


In this section, we are going to prove \cref{thres1}.
\begin{theorem}[\cref{thres1} restated]
	For every fixed $\eps > 0$ and for every $k \geq \eps\sqrt{n}$, there is an (explicitly described) algorithm running in time $n^{O(\log(\frac{1}{\eps}))}$ which almost surely finds the maximum clique in a graph $G \sim AG(n, \frac{1}{2}, k)$. The statement holds for every adversarial planting strategy (choice of $k$ vertices as a function of $G' \sim G(n, \frac{1}{2})$), and the probability of success is taken over the choice of  $G' \sim G(n, \frac{1}{2})$.
%$G$ for every possible choice of $k$ vertices by the adversary.  and  the following holds.
%	Let $G \sim AG(n, 1/2, k)$ with $k \geq \eps\sqrt{n}$.	
\end{theorem}
%The proof of \cref{thres2} is an extension of the proof for \cref{thres1}, and can be found in \cref{sec:appb}.
For now we will assume that $k = \O{\sqrt{n\log n}}$ and $k \geq 10\sqrt{n}$, the extension of the proof to any $k\geq \eps\sqrt{n}$ for arbitrary fixed $\eps > 0$ will be described in further sections.
The following theorem is key to our algorithm, and will be proved in a more general version in further sections.
\begin{theorem}\label{semitheta}
	Let $G \sim AG(n, 1/2, k)$ with $k = k(n) \geq 10\sqrt{n}$.
	Then $k \leq \vartheta(\oG) \leq k + 96\log n + 1$ with extremely high probability, for every possible choice of $k$ vertices by the adversary.
\end{theorem}



The proof of \cref{semitheta} will be given in the next section, now we will focus on proving \cref{semialgo}.
The idea is the following.
Let $K$ be the set of the vertices from the planted clique.
As known (\textbf{CITE}), the size of the maximum clique in $G(n, 1/2)$ equals $(2 + \o{1})\log n$ with extremely high probability. 
Then the size of the maximum clique in $G\sim AG(n, p, k)$ w.e.h.p. is at most $k + (2 + \o{1})\log n$, furthermore, at least $k - (2 + \o{1})\log n$ vertices of any maximum clique must belong to $K$.
On the other hand, the vertices from the maximum clique that do not belong to $K$ must have a huge neighborhood in $K$, precisely, be connected to at least $k - (2 + \o{1})\log n$ vertices from $K$.
Consequently, if we find a set $Q$ of size at most $k + \O{\log n}$, which contains at least $k - \O{\log n}$ vertices from $K$, by taking all the vertices with huge neighborhood in $Q$ we will definitely take all the vertices which belong to any maximum clique of $G$.
However, by doing so we may include too many extra vertices, which do not belong to any maximum clique but still have a huge neighborhood in $Q$.
The following proposition ensures that the number of such extra vertices will be small, for any possible set $Q$.
All assumptions for the values of $p$ and $k$ are the same as in \cref{semitheta}.
\begin{proposition}\label{neigh}
	Let $G' \sim G(n, 1/2)$, $G' = (V, E)$.
	Let $\mu/2 < \nu \leq \mu \in (0, 1]$, be arbitrary constants, and let $\alpha_\mu(n)$, $\alpha_\nu(n)$ be arbitrary (not necessary non-negative) functions of absolute value at most $\o{k}$.
	For every set $Q \subset V$ of size $\mu k + \alpha_\mu(n)$, with extremely high probability there are at most $g(n) := \frac{6}{\left(\nu - \mu/2\right)^2}\log n + 1$ vertices from $V\setminus Q$ that have at least $\nu k +  \alpha_\nu(n)$ neighbors from $Q$ in $G'$.
\end{proposition}
That is, given some set $Q$ of size at most $k + \O{\log n}$, which contains at least $k - \O{\log n}$ vertices from $K$, we can take all the vertices with at least $k - \O{\log n}$ neighbors in $Q$ and obtain a set of vertices, which has every vertex that belongs to any maximum clique of $G\sim AG(n, 1/2, k)$, plus at most $\O{\log n}$ extra vertices.
And, to find the set $Q$ yielding these properties, we will use \cref{semitheta} and compute the value of Lovasz theta function of $\oG$.
The exact process will be shown in the next subsection, we will heavily rely on the following corollary of \cref{neigh}.
\begin{corollary}\label{closeneigh}
	For every set $Q \subset V$ of size $k$, asymptotically almost sure there are at most $a(n) := 96\log n + 1$ vertices from $V\setminus Q$ with at least $\frac{3}{4}k$ neighbors from $Q$ in $G'$.
\end{corollary}
In the next section, we will prove generalizations of \cref{neigh} and \cref{closeneigh}, which immediately imply the latter.
Another useful observation is the following.
Let $J\subset K$ be an arbitrary subset of vertices from the planted clique, $|J| = \O{\log n}$.
Then, if we delete $J$ from $G$ and consider $G\setminus J$, \cref{closeneigh} and \cref{semitheta} do hold for $G\setminus J$ without any changes, as $G\setminus J$ still contains a planted clique of size $(1 - \o{1})k$.
As a result, $k - |J|\leq \vartheta(\overline{G\setminus J}) \leq k - |J| + a(n)$.



\subsection{Finding the maximum clique}

Now we are going to present the proof of \cref{semialgo}.
We use the formulation of the theta function as a geometric maximization form (\textbf{CITE})
\[\vartheta_4(\oG) = \max_{h, \{s_i\}}\sum_{i \in V}(h \cdot s_i)^2,\]
where $\{s_i \in \R^n : i \in V\}$ is an orthonormal representation of $G = (V, E)$ ($\|s_i\| = 1$ and $s_i\cdot s_j = 0 \iff (i, j) \notin E$), and $h \in \R^n$ ranges over all vectors of unit length.
We can apply semidefinite programming to solve $\vartheta_4$ within arbitrary small additive error in polynomial time, and obtain a corresponding vector $h$ and orthonormal representation $\{s_i\}$.

Suppose that we solved $\vartheta_4(\oG)$ for $G\sim AG(n, 1/2, k)$, $k \geq 10\sqrt{n}$, then by \cref{semitheta}  $k \leq \vartheta_4(\oG)\leq k + a(n)$.
It is clear that for all $i \in V$, $(h \cdot s_i)^2 \leq 1$.
We claim that there must be at most $4a(n)$ vertices $j$ from $K$ with $(h\cdot s_j)^2 < 3/4$.
Suppose the contrary, let $J \subseteq K$ be the set of all $j \in K$ with $(h\cdot s_j)^2 < 3/4$, $|J| > 4a(n)$.
Delete $J$ from the graph $G$ and consider $\vartheta_4(\overline{G\setminus J})$.
It is clear that
\[\vartheta_4(\overline{G\setminus J}) \geq \sum_{i \in V\setminus J}(h\cdot s_i)^2 = \vartheta_4(\oG) - \sum_{j \in J}(h\cdot s_j)^2,\]
hence
\begin{multline*}
\vartheta_4(\oG) \leq \vartheta_4(\overline{G\setminus J}) + \sum_{j \in J}(h\cdot s_j)^2 \leq k - |J| + a(n)  + (3/4)|J| =\\
= k + a(n) - (1/4)|J|< k + a(n) -  a(n) = k,
\end{multline*}
a contradiction.
So, there are at least $k - 4a(n)$ vertices $j \in K$ with $(h \cdot s_j)^2 \geq 3/4$.
Denote this set by $K_{3/4} \subseteq K$.

Observe that if $i \in V\setminus K$ is not connected to some $j \in K_{3/4}$, then $(h\cdot s_i)^2 \leq 1/4$.
Indeed, since $\{s_i\}$ is an orthonormal representation of $G$, $(i, j)\notin E$ implies $s_i \cdot s_j = 0$, so $(h\cdot s_i)^2 + (h\cdot s_j)^2 \leq 1$ and therefore $(h\cdot s_i)^2 \leq 1/4$.
Hence, if $i \in V\setminus K$ has $(h\cdot s_i)^2\geq 3/4$, it must be connected to the whole set $K_{3/4}$.
The set $K_{3/4}$ has size at least $k - 4a(n)$, so by \cref{neigh} there are less than $a(n)/4 + 1$ vertices $i \in V\setminus K$ with $(h\cdot s_i)^2 \geq 3/4$.
As a result, there are at most $k + a(n)/4 + 1$ vertices $i \in V$ with $(h\cdot s_i)^2 \geq 3/4$.

Let $Q$ be the set of all vertices with contribution to $\vartheta_4(\oG)$ of at least $3/4$, as shown above, $k - 4a(n) \leq |Q| \leq k + a(n)/4 + 1$ where $a(n) = 24\log n + 1$.
\begin{lemma}
	Let $i \in V\setminus Q$ be contained in some maximum clique of $G$.
	Then, with extremely high probability, $i$ must be connected to at least $k - 5a(n)$ vertices from $Q$.
\end{lemma}
\begin{proof}
	If $i \in K$, then we are done.
	Suppose that $i \in V\setminus (Q \cup K)$ belongs to some maximum clique of $G$, but has less than $k - 5a(n)$ neighbors in $Q$.
	Then, since $|Q \cap K| \geq k - 4a(n)$ and $|Q| \leq k + a(n)/4 + 1$, the number of non-neighbors of $i$ in $Q\cap K$ is greater than $a(n)/4 \geq 6\log n$. 
	Therefore, $i$ is connected to less than $k - 6\log n$ vertices from $K$.
	The maximum clique in $G$ has size at least $k$, hence the number of vertices from $V\setminus K$ in the maximum clique that $i$ belongs to is greater than $6\log n$.
	It follows that there was a clique of size at least $6\log n$ in the original $G(n, 1/2)$, which cannot happen with extremely high probability.
\end{proof}
Consequently, every vertex $i \in V\setminus Q$ that belongs to some maximum clique of $G$ must have at least $k - 5a(n)$ neighbors in $Q$.
Let $P \subset V$ be the union of $Q$ and all vertices from $V\setminus Q$ that have at least $k - 5a(n)$ neighbors from $Q$ in the graph $G$.
It is clear that $K\subseteq P$, however, we might include some additional vertices from $V\setminus (Q\cup K)$ with that many neighbors in $Q$.
By \cref{neigh} and the reasoning above, there are at most $6\log n$ vertices from $V\setminus (Q\cup K)$ that have at least $k - 5a(n)$ neighbors in $Q$.
If follows that $|P| \leq k + 12\log n + 1$.

As mentioned above, $P$ must contain all the vertices that belong to at least one maximum clique of $G$, so $P$ contains all the maximum cliques of $G$, and the maximum clique of $G[P]$, the subgraph of $G$ induced on $P$, is the maximum clique of $G$.
Moreover, $K\subseteq P$, so $P$ contains a clique of size at least $k$. 
Therefore, the minimum vertex cover of $\oG[P]$, the subgraph of $\oG$ induced on $P$, has size at most $12\log n + 1$.
Since minimum vertex cover problem is fixed-parameter tractable \cite{DF95}, we can find the minimum vertex cover of $\oG[P]$ in time $\O{2^{12\log n + 1}n} = \O{n^{14}}$ --- polynomial in $n$.
By identifying the minimum vertex cover of $\oG[P]$, we automatically find the maximum clique of $G[P]$ --- if $P'$ is the minimum vertex cover of $\oG[P]$, then $P\setminus P'$ is the maximum clique of $G[P]$.
This finishes the algorithm.

Thus, asymptotically almost sure we can find the maximum clique of $G$ in polynomial time, regardless the choice of the $k$ vertices by the adversary.
This proves \cref{semialgo}.

\subsection{Other values of $k$}

\todo[inline]{Rewrite this part w.r.t. maximum clique rather than maximum independent set}

As mentioned earlier, if $k \geq \eps\sqrt{n}$ for some constant $\eps > 0$, we apply the exactly same procedure by Alon et al., described in \cite{AKS98}.
Suppose now that $k \gg \sqrt{n\log n}$.
For this case, we introduce a new, simple algorithm, which does not require computing the Lovasz theta function.

Let $G \sim G(1/2, n)$, $G = (V, E)$, and let $k = C\sqrt{n\log n}$ for $C$ large enough (for $k \gg \sqrt{n\log n}$ the analysis is analogous).
Let $c \geq 12$ be a constant such that every vertex of $G$ has degree at least $n/2 - c\sqrt{n\log n}$ and at most $n/2 + c\sqrt{n\log n}$ with probability at least $1 - n^{-c}$.

We claim that for every $S\subseteq V$, $|S| = k$, at least $k/2$ vertices of $G[S]$ have degrees larger than $3c\sqrt{n\log n}$.
Suppose for the sake of contradiction that there is some $S\subseteq V$, $|S| = k$, and a set $S'\subset S$ of size $k/2$, such that every vertex of $S'$ has degree lower than $3c\sqrt{n\log n}$ in $G[S]$.
Consider a bipartite subgraph of $G[S]$ with parts $S'$ and $S \setminus S'$, the expected number of edges in this subgraph is $(k/2)^2\cdot (1/2) = (C^2/8)n\log n$.
On the other hand, if every vertex of $S'$ has degree smaller than $3c\sqrt{n\log n}$ in $G[s]$, there are at most $(k/2)\cdot 3c\sqrt{n\log n} = k \cdot (3cC/2)n\log n$ edges in this bipartite subgraph.
Take $C \geq 13c$, then by Chernoff, the probability of it happening is at most
\[\exp\left(-\frac{k^2c^2n\log n}{8k^2}\right) = \exp\left(-\frac{1}{8}c^2n\log n\right).\]
The total number of all possible $k/2$ by $k/2$ bipartite subgraphs of $G(1/2, n)$ is at most $\exp(6k\log n)$, so by union bound the probability that there exists the set $S$ with subset $S'$ as above is at most
\[\exp\left(6k\log n -\frac{1}{8}c^2n\log n\right) \xrightarrow{n\to\infty} 0,\]
so with extremely high probability no such subset exists, and the claim follows.

Suppose that the adversary plants an independent set of size $k$ in $G$ (which is equivalent to planting a clique), denote it by $K$.
As shown above, at least $k/2$ vertices of $K$ have degrees at least $2c\sqrt{n\log n}$ in $G[K]$, and therefore after planting the independent set on $K$, they will have degrees less than $n/2 - 2c\sqrt{n\log n}$ with high probability, and any vertex outside $K$ will have degree at least $n/2 - c\sqrt{n\log n}$.
Therefore, if we take all vertices $S$ of degree less than $n/2 - 2c\sqrt{n\log n}$, with high probability $S\subseteq K$.
By an argument similar to \cref{neigh}, if we take all vertices $Q$ that have no neighbors in $S$, with high probability $K\subseteq Q$, $|Q| \leq k + \O{\log n}$, and the subgraph induced on $Q$ contains all independent sets of maximum size.
Therefore, we can find the maximum independent set by removing the minimum vertex cover of this subgraph, which can be done in polynomial time.



==> bigk.tex <==
\section{Big values of $k$}\label{sec:bigk}

Throughout our proofs concerning the values of theta function $\vartheta(\oG)$ for  $G\sim AG(n, p, k)$, we assumed that $k = O(\sqrt{np\log n})$.
In this section, we will present a simple algorithm that, almost surely, find the maximum clique of $G\sim AG(n, p, k)$ when $k \geq C\sqrt{np\log n}$ for sufficiently large constant $C$, and $np \gg n^{2/3}\log^{1/3}n$ (when $np = O(n^{2/3}\log^{1/3}n) = O(n^{3/4})$, the algorithm from \cref{sec:constantClique} will successfully find the maximum clique for any value of $k$).

Suppose for now that $p= o(1)$.
Let $G' \sim G(n, p)$, $G' = (V, E)$, and let $s \geq 1$ be some arbitrary fixed constant.
It will be convenient for us to present the results without substituting the exact value of $s$.
By Chernoff bound, with probability at least $1 - n^{-4s}$, the degree of every every vertex $v \in V$ deviates from $np$ by at most $4s\sqrt{np\log n}$.
\begin{lemma}\label{ksubset}
    With extremely high probability, for every $K\subset V$, $|K| = k$, there are at least $k/2$ vertices $u$ from $K$, such that the degree of $u$ in $G[K]$ is less than $8s\sqrt{np \log n}$.
\end{lemma}
\begin{proof}
    Suppose for the sake of contradiction that there is some subset $K$ of $k$ vertices, with a set $K'\subset K$ of $k/2$ vertices with degrees at least $8s\sqrt{np\log n}$ in $G[K]$.
    Then the bipartite graph $B(K', K \setminus K', p)$ with parts $K'$ and $K\setminus K'$ has at least $k/2 \cdot 8s\sqrt{np\log n} = 4ks\sqrt{np\log n}$ edges.
    On the other hand, the expected number of edges in this subgraph is exactly $(k/2)^2p = k^2p/4$.
    Therefore, the probability that $B(K', K \setminus K', p)$ has at least $k^2p/3$ edges is at most $2\exp\left(-\frac{1}{72}k^2p\right)$.
    There are $\binom{n}{k} \leq 2k\log n$ possible choices of $K$, and $\binom{k}{k/2} \leq 2k\log n$ choices of subset $K'\subset K$, so the probability that there exists set $K$ for which $B(K', K\setminus K', p)$ has at least $k^2p/3$ edges is at most $2\exp\left(4k\log n -\frac{1}{72}k^2p\right)$.
    Since $k \geq C\sqrt{np\log n}$ and $p \gg \frac{\log^{1/3}n}{n^{1/3}}$, $kp \geq Cp^{3/2}\sqrt{n\log n} \gg \log n$, with extremely high probability for every possible subset $K$ of size $k$ every subset $K'\subset K$ of size $k/2$ has at most $k^2p/3$ edges in $B(K', K - K', p)$.
    
    We supposed that some set $K'$ has at least $4ks\sqrt{np\log n}$ edges in $B(K', K - K', p)$, while with extremely high probability there can be at most $k^2p/3$ edges in $B(K', K - K', p)$ for any $K, K'$.
    Therefore, if $4s\sqrt{np\log n} > kp/3 \geq Cp/3\sqrt{np\log n}$ or equivalently $C < 12s/p$, we get a contradiction.
    Hence, when $p = o(1)$, we get a contradiction for any value of constant $C$, and for every $K\subset V$, $|K| = k$, there exists $K'\subset K$, $|K'| = k/2$, such that the degrees of vertices in $K'$ in $G[K]$ are at most $8s\sqrt{np\log n}$.
\end{proof}
Suppose that subset $K\subset V$ of size $k$ is made into a clique by the adversary, and consider the subset $K'\subset K$ of $k/2$ vertices with degrees in $G[K]$ smaller than $8s\sqrt{np\log n}$.
After planting a clique on $K$, the degrees of these vertices in $G[K]$ will be $k - 1$, hence the degrees in $G$, the graph obtained from $G'$ by planting a $k$-clique on $K$, will be at least $np - 12s\sqrt{np\log n} + C\sqrt{np\log n} > np + 8\sqrt{np\log n}$ when $C \geq 20s$, with probability at least $1 - n^{-4s}$ for any choice of the adversary.
Since the degrees of $G'$ almost surely did not exceed $np + 4s\sqrt{np\log n}$, we can find $k/2$ vertices of the planted clique by taking $k/2$ vertices with highest degrees.
Then, by application of \cref{Gneigh}, among the vertices which have a large neighborhood in the set of selected vertices, there will be at most $O(\log n)$ vertices that do not belong to the planted clique, and the resulting set of vertices will almost surely contain the maximum clique of $G$.
The rest of the algorithm is the same as in \cref{sec:mainalgo}, and our success probability is at least $1 - n^{-4s}$ for the fixed number $s \geq 1$.

When $p$ is a constant ($p = \omega(1)$), our approach will be slightly different.
Let $q := 1 - p$, and consider the problem of finding a maximum independent set in $G\sim A\oG(n, p, k)$, which is equivalent to finding the maximum clique in a graph distributed by $AG(n, p, k)$.
By Chernoff bound, with probability at least $1 - n^{-4s}$, the degree of every every vertex $v \in V$ deviates from $nq$ by at most $4s\sqrt{nq\log n}$.
Let $G'\sim G(n, q)$, $G= (V, E)$.
\begin{lemma}
    With extremely high probability, for every $K\subset V$, $|K| = k$, there are at least $k / 2$ vertices $u$ from $K$, such that the degree of $u$ in $G[K]$ is greater than $8s\sqrt{nq\log n}$.
\end{lemma}
The proof is analogous to the proof of \cref{ksubset}, with only difference that we should take $C \geq \tau s$ for sufficiently large constant $\tau$, depending on constant probabilities $q$ and $p$, to make the bounds hold.
It follows that after planting an independent set on some $K\subset V$ of size $k$, the $k/2$ vertices of the resulting graph $G$ which have the smallest degrees, almost surely belong to $K$, we can consider these vertices in the complement graph (with a planted $k$-clique) and take all vertices of $\oG$ which have large neighborhood within these $k/2$ selected vertices.
The rest of the algorithm is exactly the same as the one described in \cref{sec:mainalgo}.

==> general.tex <==
\section{General case algorithm} \label{sec:general}


In this section we remove any further assumptions on the values of $p$ and $k$, except for $p < c$ for constant $c \in (0, 1)$ and $k = \Omega(\sqrt{np})$.
Thus, we complete the proof of \cref{thres1}, and extend the result to other values of $p$ and $k$.

Suppose that we would like to find the maximum clique of $G\sim AG(n, p, k)$ with $k \geq \eps\sqrt{np}$ for fixed $\eps > 0$.
Let $\zeta_c := \frac{5}{1 - c}$, and let
\[   \beta = \beta(c, \eps):= \begin{cases}
1 - (4\lceil \log_{1/p}(2\zeta_c/\eps)\rceil + 3)^{-1},& \text{if $\eps < \zeta_c$};\\
2/3,& \text{otherwise}.
\end{cases}\]
One can verify that for all values of $c$ and $\eps$, $\beta \geq 2/3$, and is upper bounded by a constant strictly less than $1$.
Denote \[  s := 2\lceil \log_{1/p}(2\zeta_c/\eps)\rceil + 2 = \frac{2 - \beta}{2 - 2\beta}.\]

If $p = O(n^{\beta - 1})$, almost surely there are no cliques of size greater than $\frac{2}{1 - \beta}= O(1)$ in $G(n, p)$, therefore we can apply the algorithm from \cref{thres2} to find the maximum clique of $G \sim AG(n, p, k)$ for any $k$ in polynomial time.
Therefore, it remains to discuss an algorithm for values of $p \gg n^{\beta - 1} = \Omega(n^{-1/3})$.

If $k \geq \zeta_c\sqrt{np}$, by applying \cref{Gsemitheta} and \cref{Gaddtheta} with $w(n) := np$, we get that for every possible choice of $k$ vertices by the adversary, with extremely high probability $k \leq \vartheta(\oG) \leq k + \frac{24}{(1 - p)^2}p\log n + 1$.
Therefore, for these values of $k$ we can apply the algorithm from \cref{sec:mainalgo}, and find the maximum clique of $G$ in polynomial time.

Suppose that $k < \zeta_c\sqrt{np}$, but we still have $k \geq \eps\sqrt{np}$.
Similar to the approach of \cite{AKS98}, we can use the algorithm that works for the case $k \geq \zeta_c\sqrt{np}$ in order to obtain the algorithm for $k \geq \eps\sqrt{np}$.
Specifically, we will ``guess'' a constant number of vertices from the planted clique, find the maximum clique in the subgraph induced on the common neighborhood of the guessed vertices, thus finding the whole maximum clique.

Let $G \sim AG(n, p, k)$, $G = (V, E)$, let $K\subset V$ be the planted $k$-clique, and let $N^*(S)$ denote the common neighborhood of vertices in $S\subset V$.
For every fixed subset $S\subset K$ of size $s$, observe that the graph $G[N^*(S)]$ behaves as $AG(|N^*(S)|, p, k - s)$.
Indeed, when $S$ is fixed, the adversary can choose $s$ vertices from $S$ and then make a clique of size $k - s$ in $G[N^*(S)]$, which is a random graph $G(|N^*(S)|, p)$.
Clearly, the cardinality of $N^*(S)$ for any fixed subset $S\subset V$ of size $s$ is a random variable with distribution $\Bin(n - s, p^s)$.
So, almost surely $|N^*(S)| = (1 + o(1))np^s$.
Note that when $w(n) := np \gg n^\beta$, $k = o(np^s)$.
Indeed, by definition of $s$, $\beta = 1 - \frac{1}{2s - 1}$, so
\[\frac{k}{np^s} = O\left(\frac{n^sw(n)^{1/2}}{nw(n)^s}\right) = O\left(\frac{n^{s - 1}}{w(n)^{s - 1/2}}\right) 
    = o\left(\frac{n^{s - 1}}{n^{(1 - 1/(2s - 1))\cdot (s  - 1/2)}}\right) = o(1).\]
Planting a clique of size $k$ can increase $|N^*(S)|$ by at most $k = o(np^s)$, so we have $|N^*(S)| = (1 + o(1))np^s$ for all $S\subset V$ almost surely, for every possible choice of adversary.

Observe that, for every sybset $S\subset V$, $|S| = s$, by our choice of $s$ we have
\[    k - s \geq \frac{\eps}{2}\sqrt{np}\geq \zeta_c\sqrt{\frac{np^s}{c}}\geq \zeta_c\sqrt{|N^*(S)|}.\]
Since $k - s \geq \zeta_c\sqrt{|N^*(S)|}$, \cref{Gsemitheta} does hold for $G[N^*(S)]$, precisely,
\[    k - s \leq \vartheta(\oG[N^*(S)]) \leq k - s + a(|N^*(S)|, p)\]
with extremely high probability, where $\oG[N^*(S)]$ is the complement graph of $G[N^*(S)]$, and function $a(n, p)$ comes from \cref{Gsemitheta}.
There are at most $n^s$ possible subsets $S\subset K$, and since the bound holds with extremely high probability, it will hold for every set $S\subset K$ of size $s$ almost surely.
Therefore, we can find the maximum clique in $G[N^*(S)]$ almost surely by applying our main algorithm described in \cref{sec:mainalgo}, for all subsets $S$ and every possible planting of the adversary.
In other words, we consider all possible $s$-subsets of all possible $k$-subsets that can be selected by the adversary, and since our bounds hold with extremely high probability, we will almost surely succeed in all cases (as for every fixed choice we have extremely high probability of success).

%Suppose that for some subsets $S\subset K$, $|S| = s$, we have $k - s = \omega(\sqrt{|N^*(S)|p\log |N^*(S)|})$.
%In this case, we can apply the algorithm from \cref{sec:bigk} to $G[N^*(S)]$, with our value of parameter $s$.
%We will find the maximum clique of $G[N^*(S)]$ with probability at least $1 - n^{-4s}$, and since there are at most $n^s$ possible subsets $S$, we will succeed on all of them with probability at least $1 - n^{-2s}$, for every possible adversarial planting.

%The number of all possible subsets $S$ is at most $n^s$, therefore applying union bound we get that for every set $S\subset V$ such that $|S| = s$ and $S\subset K$, we will find the maximum clique of $G[N^*(S)]$ with high probability, regardless of the initial choice of $K$ by the adversary.
To find the maximum clique of $G\sim AG(n, p, k)$, our initial goal, we will do the following algorithm: for every set $S\subset V$ of size $s$, consider a graph $G[N^*(S)]$ and find the maximum clique $M_S$ of $G[N^*(S)]$, using the algorithm from \cref{sec:mainalgo}.
Having tried all possible subsets $S$ of size $S$, we output the set $M_S \cup S$ such that $M_S \cup S$ is a clique and has maximum size over all sets $S$ considered.
At some point we will consider some set $S\subset K$, and the maximum clique of $G[N^*(S)]$ when combined with $S$ will give us the maximum clique of $G$.

There are at most $n^s$ possible subsets $S \subset K$, and on each subset we succeed to find the maximum clique of $G[N^*(S)]$ with extremely high probability for every possible planting.
As a result, with extremely high probability, we will find the maximum clique of $G$ regardless the choice of adversary.
This completes the description of the algorithm, proving the generalization of \cref{thres1}.




==> hardness.tex <==
\section{Hardness}\label{sec:hardnessproof}

In this section, we are going to prove \cref{thres3}.
%It will be convenient to consider planted independent set problem instead of the planted clique problem.
%\begin{definition}
%    We say that graph $G$ on $n$ vertices has distribution $\oG(n, p, k)$, if its complement $\oG$ has distribution $G(n, 1 - p, k)$.
%    Similarly, $G\sim A\oG(n, p, k)$, if $\oG \sim AG(n, 1-p, k)$.
%\end{definition}
%That is, $G \sim \oG(n, p, k)$, if $G$ is formed by planting a random independent set of size $k$ in $G(n, p)$, while $G\sim A\oG(n, p, k)$ if the independent set in $G(n, p)$ was planted by the adversary.
%When $G \sim A\oG(n, p, k)$, we say that $G$ has adversarially planted independent set of size $k$. 
\begin{theorem}[\cref{thres3} restated]\label{hardness}
    For every $\delta, \gamma \in (0, 1)$ the following holds.
    Let $G \sim A\oG(n, p, k)$ with $p = n^{\delta - 1}$ and $5n^{1 - \delta}\log n \leq k \leq n - 2n^{\delta + \rho}$ for $0 < \rho < (1-\delta)/2$.
    If there exists a randomized polynomial time algorithm that finds an independent set of size at least $k$ in $G$ with probability at least $\gamma$ (over the distribution $G(n, p)$ and the randomness of the algorithm), then $RP = NP$.
\end{theorem}

We first present the high-level idea of the proof.
Let $\Aa$ be the algorithm as in \cref{hardness}, and let $H = (M, E_H)$ be an  $m$-vertex graph for which finding a maximum independent set is NP-hard, we choose $m$ so that $m \ll k \leq n$.
We will show that we can use $\Aa$ to find the maximum independent set in $H$.
Let $G_H = (V, E)$ be a graph on $n$ vertices obtained as follows: we add $n - m$ additional isolated vertices to $H$, and for every pair of vertices $u, v$ where $u \in V$ and $v \in V\setminus M$ we draw an edge $(u, v)$ with probability $p$.
%It is clear that $G_H \sim G(n, p, H)$ for some particular fixed partition of $n$ vertices into $m$ disjoint subsets.
Let $k' < m$ be the size of maximum independent set of $H$.
Among the common non-neighbors of $M$ in $G_H$, we select a random subset $I'$ of size $k - k'$ and make it into an independent set, obtaining the graph $\wG_H$ (we will later assure that we the common non-neighborhood of $M$ is big enough).
The maximum independent set of the resulting graph $\wG_H$ has size at least $k$, since $\wG_H$ contains an independent set of size $k$, which can be obtained by combining the planted independent set $I'$ of size $k - k'$ and the maximum independent set of size $k'$ in $H$.

Note that the graph $\wG_H$ can be obtained from $G_H$ by planting an independent set of size $k$, we should choose any maximum independent set of $H$ and select $k - k'$ vertices randomly among the non-neighbors of $H$, thus choosing $I'$.
On the other hand, for any graph $G \sim A\oG(n, p, k)$, algorithm $\Aa$ would find the maximum independent set of $G$ with constant probability.
We will show that, for a carefully chosen graph $H$,
\begin{enumerate}[label=(\roman*)]
    \item  the distribution of $\wG_H$ is \textit{statistically close} to $A\oG(n, p, k)$.
    That is, for every fixed instance of $\wG_H$, the probability of obtaining $\wG_H$ via the process above differs from the probability of obtaining $\wG_H$ via sampling from $A\oG(n, p, k)$ at most by a constant factor;
    \item with high probability, for every independent set $I$ of $\wG_H$, $I$ is a maximum independent set of $\wG_H$ if and only if it has size exactly $k$ and $I = I_H \cup I'$, where $I_H$ is some maximum independent set of $H$.
\end{enumerate}
If both (i) and (ii) hold, since $\Aa$ succeeds to find an independent set of size at least $k$ in $G \sim A\oG(n, p, k)$ with constant probability, it will successfully find a maximum independent set of $\wG_H$ of size $k$ with constant probability.
Then we can find the maximum independent set $I_H$ of $H$ as follows: construct multiple instances of $\wG_H$ from $H$ and give them as an input to $\Aa$, until it returns the some independent set $I$ of size exactly $k$.
The probability of the latter event is at least constant, therefore the whole process will take polynomial expected time.
Since we know by construction which vertices of $\wG_H$ do belong to $H$, and $I = I_H \cup I'$, we will be able to determine the maximum independent set $I_H$ of $H$ itself.

Now we will give the complete proof.
We start by describing the particular family of graphs $H$ that we use in the construction above.
\begin{definition}
	Given a graph $H$, denote its average degree by $\alpha$.
	A graph $H$ is balanced if every induced subgraph of $H$ has an average degree at most $\alpha$.
\end{definition}
\begin{theorem}\label{nph}
	For any $0 < \eta \leq 1$, finding the maximum independent set in a balanced graph with average degree $2 < \alpha < 2 + \eta$ is NP-hard.
\end{theorem}
\begin{proof}
	It is well known that finding the maximum independent set in 3-regular graphs is NP-hard.
	Therefore, it is enough to show that there exists a polynomial time reduction $\Rr$ such that for any given 3-regular graph $H$ it holds that 
	\begin{itemize}
		\item $\Rr(H)$ is a balanced graph with an average degree $2 < \alpha < 2 + \eta$,
		\item Given the maximum independent set of $\Rr(H)$ one can find the maximum independent set of $H$ in polynomial time.
	\end{itemize}
	
	Let $H$ be a 3-regular graph with maximum independent set of size $k$.
	The graph $H'$ is constructed as follows: take an arbitrary edge $(u, v)$ of $H$ and double-subdivide it, adding two vertices $u'$, $v'$ to this edge, resulting in a path $(u, u', v', v)$.
	It is easy to check that the maximum independent set of $H'$ has size exactly $k + 1$, and there exists an independent set of size $k + 1$ which includes one of the two added vertices.
	Moreover, if none of $u'$, $v'$ was included, then both $u$ and $v$ must be included in the maximum independent set of $H'$, but then we can replace $u$ by $u'$ or $v$ by $v'$, so w.l.o.g. we can assume that the maximum independent set of $H'$ has either $u'$ or $v'$ included.
	
	We will use this observation to construct a reduction $\Rr(H)$ for the 3-regular graph $H$ on $2n$ vertices.
	We do the following: each edge is subdivided $2t$ times, where $t$ is the parameter we choose later.
	There are $3n$ edges in $H$, so by doing so we add $2t \cdot 3n$ vertices of degree $2$.
	Then the average degree of the resulting graph $\Rr(H)$ is
	\[    \alpha = \frac{2t \cdot 3n \cdot 2 + 2n \cdot 3}{2t \cdot 3n + 2n} = \frac{6t + 3}{3t + 1} = 2 + \frac{1}{3t + 1},\]
	which is at most $3$ (setting $t = 0$).
	To make $1/(3t + 1) < \eta$ we should take $t > \frac{1}{3}(\frac{1}{\eta} - 1)$, and the average degree of $\Rr(H)$, $\alpha$, is greater than $2$ and less than $2 + \eta$.
	
	The graph $\Rr(H)$ is balanced.
	To see this, consider a subset $S^*\subseteq \Rr(H)$ such  that the average degree on the induced subgraph $\Rr(H)[S^*]$ is maximized to $\alpha^*$.
	W.l.o.g., we can assume that $\Rr(H)[S^*]$ is connected and has at least 2 vertices (so $\alpha^* > 1$).
	Observe that each subgraph of maximum average degree has minimum degree at least 2: if $v$ is the vertex of degree $1$ in $\Rr(H)[S^*]$, then the average degree of $\Rr(H)[S^*\setminus v]$ is strictly greater than the one of $\Rr(H)[S^*]$.
	
	Let $x$ and $y$ be the numbers of vertices of $\Rr(H)[S^*]$ with degree 2 and 3 respectively.
	Then 
	\[       \alpha^* = \frac{2x + 3y}{x + y} = 2 + \frac{y}{x + y}.\]
	The vertices of degree 3 are exactly the vertices of the original graph $H$.
	Hence, if we want to increase $y$, we should connect two vertices $i \neq j$ of degree 2 by a path of length $2t\cdot d_H(i, j)$, where $d_H(i, j) \geq 1$ is the distance between $i$ and $j$ in $H$, which would require adding at least $2t\cdot d_H(i, j)$ vertices of degree $2$, thus increasing $x$.
	It follows that the expression for $\alpha^*$ will reach its maximum value if and only if $\Rr(H)[S^*] = \Rr(H)$, so $\Rr(H)$ is a balanced graph.
	
	Suppose that we are given the maximum independent set of $\Rr(H)$.
	By the reasoning above, its size will be exactly $3n \cdot nt$ plus the size of the maximum independent set of $H$, and every path of length $2nt$ between two vertices of degree 3 has exactly $nt$ vertices in the maximum independent set of $\Rr(H)$.
	Then, we can simply scan all the vertices in the given independent set and remove all the vertices of degree 2, which will give us the maximum independent set of $H$.
	The theorem follows.
\end{proof}

For the rest of the section we will assume that $H$ is a balanced graph with average degree $2 < \alpha < 2 + \eta$ with $\eta := \min(\frac{2}{1/\delta - 1}, 1)$, where $\delta$ comes from \cref{hardness}.

In order to show that the distribution of $\wG_H$ (from the construction above) for this family of graphs $H$ is statistically close to $A\oG(n, p, k)$, we need to prove that the process of constructing $\wG_H$ can be imitated by the adversary.
%Specifically, we want to show that given graph $G(n, p)$, adversary can find a copy of $H$ in it, select $k - k'$ vertices from its common non-neighborhood, and make them into an independent set, resulting in a graph from $A\oG(n, p, k)$, where $\Aa$ can find an independent set of size at least $k$ with constant probability.
%However, not every instance of $G(n, p)$ contains $H$ as a vertex-induced subgraph.
We are going to show that the probability measure of graphs $G' \sim G(n, p)$ containing many copies of $H$ as vertex induced subgraphs is high enough, which will assure that for a large portion of graphs $G'\sim G(n, p)$, the adversary can select a copy of $H$ in $G'$ and plant an independent set of size $k$, imitating the construction of $\wG_H$.
%, and since $\Aa$ succeeds on most of the graphs from $A\oG(n, p, k)$, it should succeed on $\wG_H$ with large enough probability.

To give a formal proof, we will need some additional definitions.
Let $G$ be an $n$-vertex graph, and let $m \leq n$ be an integer, assume that $m$ divides $n$.
Consider a fixed partition of the vertex set of $G$ into $m$ disjoint subsets of vertices, each of size $n/m$.
A vertex set $S$ of size $m$, such that for each of the $m$ parts there is exactly one vertex in $S$ belonging to this part, is said to \textit{obey the partition}.
\begin{definition}
    Let $H$ be an arbitrary $m$-vertex graph, and let $G' \sim G(n, p)$ be a random graph $n \geq m$ vertices, $p \in (0, 1)$.
    Consider the fixed partition of the vertex set of $G'$ into $m$ disjoint subsets.
    We say $G$ is distributed by $G(n, p, H)$, if it is created by the following random process.
    \begin{enumerate}
        \item Choose a random subset $M$ of $m$ vertices from $G'$ that obeys the partition.
        \item Replace the induced subgraph of $G'$ on $M$ by the graph $H$.
    \end{enumerate}
    When $G\sim G(n, p, H)$, we say that $H$ was randomly planted in $G(n, p)$.
\end{definition}
This distribution is equivalent to the following.
Take $n$ isolated vertices and consider their fixed partition into $m$ disjoint subsets.
Then, select a random subset $M$ of $m$ vertices that obeys the partition, and create $H$ on $M$.
Next, for every pair of vertices $u, v$ where $u \in V$ and $v \in V\setminus M$, draw an edge $(u, v)$ with probability $p$, thus completing $H$ to a random graph with a planted $H$.
Note that this is exactly the same procedure as the construction of graph $G_H$ we discussed earlier, where we added $n - m$ isolated vertices to $H$ and then draw random edges.
We will consider graphs $H$ such that every vertex $i \in [m]$ of $H$ will be required to come from part $i$ (we just fix such partition that this property holds for the graph $H$ in consideration).

For the given graph $G$, let $X_H(G)$ be the number of sets $S$ of size $m$ obeying the partition, such that the subgraph of $G$ induced on $S$ is $H$.
%Let $C_H(G)$ be the number of induced subgraphs of $G$ that are isomorphic to $H$, such that they obey the partition.
For random $G$ number, $X_H(G)$ is a random variable.
Denote by $p(G)$ the probability to output $G$ according to $G(n, p)$, and by $p_H(G)$ the probability to output $G$ according to $G(n, p, H)$.
Further below, we establish the relationship between $p(G)$ and $p_H(G)$, which will be used to prove \cref{lem:closeStatistics}.
\begin{lemma}\label{prob}
	For any given graph $G$ it holds that $p_H(G) = \frac{X_H(G)}{\E{X_H(G)}}p(G)$.
\end{lemma}
\begin{proof}
	Let $e$ be the number of edges in $G$ and consider $p_H(G)$.
	Out of the $\left(\frac{n}{m}\right)^m$ options to choose a subset $M$ in $G(n, p, H)$, only $X_H(G)$ options are such that the subgraph induced on $M$ is $H$, so that the resulting graph could be $G$.
	Since $H$ has average degree $\alpha$, it has exactly $\alpha m / 2$ edges.
	Note that 
	\[     \E{X_H(G)} = \left(\frac{n}{m}\right)^mp^{\frac{\alpha m}{2}}(1 - p)^{\binom{m}{2} - \frac{\alpha m}{2}}.\]
	Given that we chose a suitable $M$, the rest of the edges $(e - \frac{\alpha m}{2})$ of $G(n, p, H)$ should agree with $G$.
	It follows that 
	\begin{multline*}
	p_H(G) = \frac{X_H(G)}{\left(\frac{n}{m}\right)^m}p^{e - \frac{\alpha m}{2}}(1 - p)^{\binom{n}{2}- \left(\binom{m}{2} + e - \frac{\alpha m}{2}\right)} = \\
	= \frac{X_H(G)}{\left(\frac{n}{m}\right)^mp^{\frac{\alpha m}{2}}(1 - p)^{\binom{m}{2} - \frac{\alpha m}{2}}}p^e(1 - p)^{\binom{n}{2} - e} = \\=\frac{X_H(G)}{\E{X_H(G)}}p^e(1 - p)^{\binom{n}{2} - e} = \frac{X_H(G)}{\E{X_H(G)}}p(G).
	\end{multline*}
\end{proof}
Recall that algorithm $\Aa$ succeeds to find an independent set of size at least $k$ in $A\oG(n, p, k)$ with probability at least $\gamma$.
Then, the probability measure of graphs from $G(n, p)$ where $\Aa$ finds an independent set of size at least $k$ with respect to \textit{all} possible plantings with probability at least $\gamma/2$ is at least $\gamma/2$, this holds by averaging (consider the adversary that tries all possible plantings and simulates $\Aa$ on resulting graphs, then choosing the input where $\Aa$ fails with highest probability over the randomness of $\Aa$).
Suppose that for some constant $\tau$ we have $p_H(G) \geq \tau p(G)$ for all graphs $G$.
Then, the probability measure of graphs from $G(n, p, H)$ where $\Aa$ finds an independent set of size at least $k$ with respect to \textit{all} possible plantings with probability at least $\gamma/2$ is at least $\tau\gamma/2$.
This will imply that $\Aa$ will successfully find an independent set of size at least $k$ in $\wG_H$ at least with some constant probability, and we are halfway done.

There exists no universal constant $\tau$ such that $p_H(G) \geq \tau p(G)$ for all $G$, as $G$ can simply not contain any copy of $H$.
Instead, we will find a constant $\tau$ such that, for specific family of graphs $H$, a large portion of graphs $G \sim G(n, p)$ do have $X_H(G) \geq \tau \E{X_H(G)}$.
By \cref{prob} we get that for many graphs $G$ the inequality $p_H(G) \geq \tau p(G)$ does hold (thus proving \cref{lem:closeStatistics}).
%Since $C_H(G) \geq X_H(G)$, it suffices to find a constant $\tau$ such that $X_H(G) \geq \tau \E{C_H(G)}$ with large enough constant probability.
\begin{theorem}\label{copy}
    Let $0 < \eps < 1/7$ be a constant, and let $G \sim G(n, p)$ be a random graph with $p \in (0, 1)$.
    Let $H$ be arbitrary balanced graph with average degree $2 < \alpha < 3$ on $m$ vertices.
	If $m$ satisfies $\eps \geq m^2p$ and $\eps^2 \geq \frac{m^4}{n^2p^\alpha}$, then for every $\beta \in [0, 1)$
	\[     \P{X_H(G) \leq \beta\E{X_H(G)}} \leq \frac{4\eps}{(1 - \beta)^2}.\]
\end{theorem}
\begin{proof}	
    Let $w(n) := np$, so $p = w(n)/n$.
	%We are going to prove the inequality by proving the following two statements:
	%\begin{itemize}
	%	\item[(i)] $\E{X_H(G)} \leq \E{C_H(G)} \leq \frac{1}{1 - \eps}\E{X_H(G)}$;
	%	\item[(ii)] $\P{X_H(G) > \beta\E{X_H(G)}} \geq 1 - \frac{4\eps}{(1 - \beta)^2}$.
	%\end{itemize}
	%It is easy to see that combining (i) and (ii) gives us the desired probability bound.
	Let $Y_H(G)$ be a random variable counting the number of sets $S$ obeying the partition that have $H$ as an edge induced subgraph of $G$, but may have additional internal edges.
	By definition, $X_H(G) \leq Y_H(G)$ and
	\[   \E{Y_H(G)} = \left(\frac{n}{m}\right)^mp^{\frac{\alpha m}{2}} = \left(\frac{n}{m}\right)^m\cdot \left(\frac{w(n)}{n}\right)^{\frac{\alpha m}{2}} = \left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{\frac{m}{2}}.\]
	A set $S$ in $Y_H(G)$ contributes to $X_H(G)$ if it has no internal edges beyond those of $H$.
	This happens with probability 
	\[   (1 - p)^{\binom{m}{2} - \frac{\alpha m}{2}} \geq 1 - \binom{m}{2}\frac{w(n)}{n} \geq 1 - \frac{m^2w(n)}{n} \geq 1 - \eps,\]
	so
	\[   \E{X_H(G)} \geq (1 - p)^{\binom{m}{2} - \frac{\alpha m}{2}}\E{Y_H(G)} \geq (1 - \eps)\E{Y_H(G)}.\]
	
	Note that if $\E{Y_H(G)^2} \leq (1 + \eps)\E{Y_H(G)}^2$, the inequality above gives us $\E{X_H(G)^2} \leq \frac{1 + \eps}{(1 - \eps)^2}\E{X_H(G)}^2$.
	We will now compute $\E{Y_H(G)^2}$.
	Given the occurrence of $H$, consider another potential occurrence $H'$ that differs from it by $t$ vertices.
	Since $H$ is balanced graph,
	\[|E(G[H'\setminus H])| + |E(G[H'\setminus H], G[H])| \geq \frac{\alpha |V(G[H'])|}{2} - \frac{\alpha|V(G[H\cap H'])|}{2} \geq \frac{\alpha t}{2}.\]
	Hence, the conditional probability that $H'$ realized is at most $p^{\frac{\alpha t}{2}}$.
	The number of ways to choose $t$ other vertices is $\binom{m}{t}\left(\frac{n}{m}\right)^t$ (first choose $t$ groups out of $m$ in the partition, then choose one vertex in each group).
	Hence, the expected number of such occurrences is 
	\[    \mu_t \leq \binom{m}{t}\left(\frac{n}{m}\right)^tp^{\frac{\alpha t}{2}} = \binom{m}{t}\left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{\frac{t}{2}}. \]
	It follows that $\mu_m \leq \E{Y_H(G)}$.
	Moreover,
	\[ \sum_{t = 1}^{m/2}\frac{\mu_t}{\E{Y_H(G)}} \leq \sum_{t = 1}^{m/2}\binom{m}{t}\left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{\frac{t - m}{2}} \leq 2^m\left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{-\frac{m}{4}} = \left(\frac{16m^2n^{\alpha - 2}}{w(n)^{\alpha}}\right)^{\frac{m}{4}}.\]
	Furthermore,
	\[  \sum_{t  = m/2}^{m - 1}\frac{\mu_t}{\E{Y_H(G)}} \leq \sum_{t = m/2}^{m - 1}m^{m - t}\left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{\frac{t - m}{2}} = \sum_{t  = m/2}^{m - 1}\left(\frac{w(n)^{\alpha}}{m^4.n^{\alpha - 2}}\right)^{\frac{t - m}{2}}.\]
	when $w(n)^\alpha \geq 2m^4n^{\alpha - 2}$ the term $t = m - 1$ dominates, and hence the sum is at most roughly $\sqrt{\frac{m^4n^{\alpha - 2}}{w(n)^{\alpha}}}$.
	Since $\eps^2 \geq \frac{m^4n^{\alpha  - 2}}{w(n)^\alpha}$ we have 
	\begin{multline*}
	    \sum_{t = 1}^{m  - 1}\frac{\mu_t}{\E{Y_H(G)}} \leq \left(\frac{16m^2n^{\alpha - 2}}{w(n)^{\alpha}}\right)^{\frac{m}{4}} + (1 + o(1))\sqrt{\frac{m^4n^{\alpha - 2}}{w(n)^{\alpha}}} \leq \\
	    \leq (1 + o(1))\sqrt{\frac{m^4n^{\alpha - 2}}{w(n)^{\alpha}}} \leq \eps
	\end{multline*}
	and $\sum_{t = 1}^m\mu_t \leq (1 + \eps)\E{Y_H(G)}$.
	Hence can bound $\E{Y_H(G)^2} \leq \E{Y_H(G)}\sum_{t = 1}^m\mu_t \leq (1 + \eps)\E{Y_H(G)}^2$, and
	%Recall that $X_H(G) \leq Y_H(G)$ and $\E{X_H(G)} \geq (1 - \eps)\E{Y_H(G)}$.
	%Then
	\[\E{X_H(G)^2} \leq \E{Y_H(G)^2} \leq (1 + \eps)\E{Y_H(G)}^2 \leq \frac{1 + \eps}{(1 - \eps)^2}\E{X_H(G)}^2 \leq (1 + 4\eps)\E{X_H(G)}^2.\]
	The last inequality holds since $\eps < 1/7$.
	We get that $\V{X_H(G)} = \E{X_H(G)^2} - \E{X_H(G)}^2 \leq 4\eps\E{X_H(G)}^2$.
	By Chebyshev's inequality we conclude that
	\begin{multline*}
	    \P{X_H(G) \leq \beta\E{X_H(G)}} = \P{X_H(G) \leq \E{X_H(G)} - (1 -\beta)\E{X_H(G)}} \leq\\\leq  \frac{\V{X_H(G)}}{(1 - \beta)^2\E{X_H(G)}^2}\leq \frac{4\eps}{(1 -\beta)^2},
	\end{multline*}
	as desired.
\end{proof}
Combining \cref{prob} with \cref{copy} we manage to prove \cref{lem:manyH}.
\begin{corollary}\label{subcopy}
	For every $0 < \delta < 1$ and $0 < \eps < 1/7$ there exists some $\rho > 0$ such that the following holds for large enough $n$.
	Let $G \sim G(n, p)$ be a random graph with $p = n^{\delta - 1}$.
	If a balanced graph $H$ on $m$ vertices with average degree $\alpha$ satisfies $2 < \alpha < \min(2 + \frac{2}{1/\delta - 1}, 3)$ and $m = n^{\rho}$, then $\E{X_H(G)}\xrightarrow{n\to\infty}+\infty$, and for every $\beta \in [0, 1)$
	\[     \P{X_H(G) \leq \beta\E{X_H(G)}} \leq \frac{4\eps}{(1 - \beta)^2}.\]
\end{corollary}
\begin{proof}
    Let $w(n) := np$, so $p = w(n)/n$.
	Observe that there exists some $\rho > 0$ such that for large enough $n$ we have 
	\[   \eps \geq \frac{m^2w(n)}{n} = n^{2\rho + \delta - 1},\]
	just choose $\rho < (1 - \delta)/2$.
	Moreover, there exists some $\rho > 0$ such that for large enough $n$ we have 
	\[  \eps^2 \geq \frac{m^4n^{\alpha  - 2}}{w(n)^\alpha} = n^{4\rho + \alpha(1 - \delta) - 2}.\]
	Indeed, since $2 < \alpha < 2 + \frac{2}{1/\delta - 1}$, we have $\alpha(1 - \delta) < 2$, so for $\rho < (2 - \alpha(1 - \delta))/4$ the inequality holds for large $n$.
	Take $\rho < \min((1 - \delta)/2, (2 - \alpha(1 - \delta))/4)$, and by applying \cref{copy} we prove the probability bound.
	Equivalently, set 
	\[   m = \min\left\{\sqrt{\eps}n^{\frac{1 - \delta}{2}}, \sqrt{\eps}n^{\frac{2 - \alpha(1 - \delta)}{4}}\right\}.\]
	
	To show that $\E{X_H(G)}\xrightarrow{n\to\infty}+\infty$, recall from the proof of \cref{copy} that 
	\[   \E{X_H(G)}\geq (1 - \eps) \left(\frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}}\right)^{\frac{m}{2}}.\]
	As $w(n) = n^\delta$ and $m = n^\rho$,
	\[  \frac{w(n)^{\alpha}}{m^2n^{\alpha - 2}} = n^{-2\rho - \alpha(1 - \delta) + 2}.\]
	Since $\rho < (2 - \alpha(1 - \delta))/4$, $2 - \alpha(1 - \delta) - 2\rho > 2\rho$, so $\E{X_H(G)} \geq (1 - \eps)n^{m\rho} \xrightarrow{n\to\infty}+\infty$.
\end{proof}
\begin{corollary}\label{goodmes}
    Let $k \geq \Omega(n^{1 - \delta})$ be arbitrary.
    Let $p = p(n) = n^{\delta - 1}$ for $0 < \delta < 1$, and let $\Aa$ be an algorithm that finds an independent set of size at least $k$ in $A\oG(n, p, k)$ with probability at least $\gamma \in (0, 1)$.
    Let $H$ be an arbitrary balanced graph with average degree $2 < \alpha < \min(2 + \frac{2}{1/\delta - 1}, 3)$ on $m$ vertices, where
    \[   m = \min\left\{\sqrt{\eps}n^{\frac{1 - \delta}{2}}, \sqrt{\eps}n^{\frac{2 - \alpha(1 - \delta)}{4}}\right\}.\]
    Let $G_H \sim G(n, p, H)$, and suppose that the adversary plants an independent set of size $k$ in $G_H$.
    The probability measure with respect to $G(n, p, H)$ of graphs $G_H$, such that $\Aa$ succeeds to find an independent set of size at least $k$ for with probability at least $\gamma / 2$ for every possible adversarial planting, is at least $\gamma/20$.
\end{corollary}
\begin{proof}
    Observe that the probability measure of graphs from $G(n, p)$ where $\Aa$ finds an independent set of size at least $k$ with respect to \textit{all} possible adversarial plantings with probability at least $\gamma/2$ is at least $\gamma/2$, this holds by averaging (consider the adversary that tries all possible plantings and simulates $\Aa$ on resulting graphs, then choosing the input where $\Aa$ fails with highest probability over the randomness of $\Aa$).

    Take $\eps = \gamma/100$ and apply \cref{subcopy}.
    For every $\beta \in [0, 1)$,
    \[ \P[G\sim G(n, p)]{X_H(G) \leq \beta\E{X_H(G)}} \leq \frac{4\eps}{(1 - \beta)^2}.\]
	Set $\beta$ to be such that $\beta \geq 1/5$ and $\frac{4\eps}{(1 - \beta)^2} \leq \gamma/4$.
	Therefore the probability measure of graphs $G$ from $G(n, p)$ where $\Aa$ finds the independent set of size at least $k$ with probability at least $\gamma /2$ (over the randomness of $\Aa$), for every possible adversarial planting, and that have $X_H(G) \geq \beta\E{X_H(G)}$, is at least $\gamma/4$.
	
	By \cref{prob}, for every $G \sim G(n, p)$ with $X_H(G) \geq \beta\E{X_H(G)}$ we have 
	\[  p_H(G) = \frac{X_H(G)}{\E{X_H(G)}}p(G) \geq \frac{\beta\E{X_H(G)}}{\E{X_H(G)}}p(G) = \beta p(G), \]
	thus proving \cref{thm:closeStatistics}.
	It follows that the probability measure with respect to $G(n, p, H)$ of graphs $G_H$, such that $\Aa$ succeeds to find an independent set of size at least $k$ for with probability at least $\gamma / 2$ for every possible adversarial planting, is at least $\beta\cdot \gamma/4 \geq \gamma/20$.
\end{proof}

To finish the proof of \cref{hardness}, we will also need the following simple lemma.
\begin{lemma}\label{nonneigh}
    Let $\delta \in (0, 1)$ and $0 < \rho < (1-\delta)/2$.
    Let $G \sim G(n, p)$ be a random graph with $p = n^{\delta - 1}$.
    For every set $S$ of $n^{\rho}$ vertices of $G$ the size of the common non-neighborhood of $S$ is at least $n - 2n^{\delta + \rho}$ with probability at least $1 - \exp(-\frac{1}{4}n^{\delta})$.
\end{lemma}
\begin{proof}
    We clearly have $\rho + \delta < 1$.
    By Chernoff bound, the maximum degree of $G$ is at most $2n^{\delta}$ with probability at least $1 - \exp(-\frac{1}{4}n^{\delta})$.
    Hence, any set $S$ of $n^{\rho}$ vertices has at most $2n^{\delta + \rho}$ neighbors.
    Then, for any set $S$ of this size the common non-neighborhood of $S$ has size at least $n - 2n^{\delta + \rho}$ with probability at least $1 - \exp(-\frac{1}{4}n^{\delta})$.
\end{proof}

Recall the construction of graph $\wG_H$.
We are given a graph $H = (M, E_H)$ on $m = n^{\rho}$ vertices, that satisfies \cref{goodmes}, and let $k$ satisfy $5n^{1 - \delta}\log n \leq k \leq n - 2n^{\delta + \rho}$.
Note that $m \ll k \leq n$.
Let $G_H = (V, E)$ be a graph on $n$ vertices obtained as follows: we add $n - m$ additional isolated vertices to $H$, and for every pair of vertices $u, v$ where $u \in V$ and $v \in V\setminus M$ we draw an edge $(u, v)$ with probability $p$.
As was mentioned, $G_H \sim G(n, p, H)$ for a particular fixed partition of $n$ vertices into $m$ disjoint subsets.
Let $k' < m$ be the size of maximum independent set $I_H$ of $H$.
Among the common non-neighbors of $M$ in $G_H$, we select a random subset $I'$ of size $k - k'$ and make it into an independent set, obtaining the graph $\wG_H$, by \cref{nonneigh} there will be enough non-neighbors with exponentially high probability.
Let $I$ be a maximum independent set of the resulting graph $\wG_H$, it has size at least $k$, since $\wG_H$ contains an independent set of size $k$, which can be obtained by combining the planted independent set $I'$ of size $k - k'$ and the maximum independent set $I_H$ of size $k'$ in $H$.
It is easy to see that every graph $\wG_H$ can be obtained via planting of the independent set of size $k$ in $G_H$ distributed by $G(n, p, H)$.
Therefore, by \cref{goodmes}, algorithm $\Aa$ successfully finds an independent set of size at least $k$ in $\wG_H$ with probability at least $\gamma^2/40$, over the randomness of $\Aa$ and the distribution $G(n, p, H)$.

It remains to show that, with high probability, the independent set that $\Aa$ finds given $\wG_H$ has size exactly $k$ and is equal to a maximum independent set $I$ of $\wG_H$ which has the form $I = I_H \cup I'$ for a maximum independent set $I_H$ of graph $H$.
We will need the following lemmas.
\begin{lemma}
	With probability at least $1 - \exp(-\frac{1}{2}n^{1 - \delta}\log^2 n)$, there is no independent set of size $k - k'$ in $G_H[V\setminus M]$.
\end{lemma}
\begin{proof}
	By first moment method the probability that there exists an independent set of size $t$ is at most
	\begin{multline*}
	    \binom{n}{t}(1 - p)^{\frac{t(t - 1)}{2}} \leq \exp\left(t\log n + t - t\log t -\frac{t(t - 1)}{2}n^{\delta - 1}\right) =\\= \exp\left(\log n + 1 - \log t - \frac{t - 1}{2}n^{\delta - 1}\right)^t,
	\end{multline*}
	which for $t \geq k - k' \geq 2n^{1 - \delta}\log n$ is at most $\exp(-\frac{1}{2}n^{1 - \delta}\log^2 n)\xrightarrow{n\to\infty}0$.
\end{proof}
\begin{lemma}
	For every integer $t \geq 1$, with probability at least $1 - 3/n$ every subset $Q \subset V\setminus (M\cup I')$ of vertices of graph $G_H[V\setminus M]$, $|Q| = t < k - k'$, has at least $t + 1$ neighbors in $I'$. 
\end{lemma}
\begin{proof}
    To prove this, view the process of generating $\wG_H$ in a following way.
	Initially, we have the graph $H$ and $n - m$ isolated vertices.		Then, for every pair of vertices $u, v$ where $u \in M$ and $v \in V\setminus M$, draw an edge $(u, v)$ with probability $p$.
	By doing so, we determine the set $W\subseteq V\setminus M$ of vertices that have no neighbors in $H$.
	Select a random subset $I' \subset W$ of size $k - k'$, and for every pair of vertices from $V\setminus M$ which both do not belong to $I'$, draw an edge with probability $p$.
	It is clear that the degree of every vertex in $G_H[V\setminus (M \cup I')]$ is a random variable distributed as $\Bin(n - m, p)$.
		
	Fix a particular set $Q \subset V\setminus (M\cup I')$ and suppose that it has at most $t$ neighbors in $I'$.
	The probability of the latter happening, by Chernoff bound, is at most $2\exp(-\frac{1}{2}t(k - k')p) \leq 2\exp(-\frac{5}{2}t\log n)$.
	There are $\binom{n}{t} \leq \exp(t\log n + t)$ possible sets $Q$, so by union bound the probability that some subset $Q\subset V\setminus (M\cup I')$ of size $t$ has at most $t$ neighbors in $I'$ is at most $2\exp(-t\log n)$.
	Then the probability of this happening for any value $t < k - k'$ is at most
	\[    2\sum_{t = 1}^{k - k' - 1}n^{-t} \leq \frac{3}{n}.\]
	The lemma follows.
\end{proof}
Combining these two lemmas we get that with probability at least $1 - 4/n$ the randomly planted set $I'$ in the non-neighborhood of $M$ in $G_H$ is the unique maximum independent set of $\wG_H[V\setminus M]$.
Observe that the size of any maximum independent set $I$ of $\wG_H$ is at most $k$, which implies $|I| = k$.
Otherwise, $I$ must contain at least $k - k' + 1$ vertices from $V\setminus M$, which is not possible, as the size of the maximum independent set in $\wG_H[V\setminus M]$ is $k - k'$.
By the same reasoning, for some maximum independent set $I_H$ of $H$, set $I$ must contain whole $I_H$.		
As a result, with probability at least $1 - 4/n \geq \gamma / 40$ the size of the maximum independent set in $\wG_H$ is exactly $k$, and any independent set $I$ of size $k$ in $\wG_H$ has the form $I = I_H \cup I'$, where $I_H$ is some maximum independent set of $H$.
	
Consider graph $G_H \sim G(n, p, H)$, such that algorithm $\Aa$ succeeds to find an independent set of size at least $k$ with probability at least $\gamma / 2$ for every possible adversarial planting of an independent set of size $k$, the probability measure of such graphs with respect to $G(n, p, H)$ is at least $\gamma / 20$.
For every such graph $G_H$, if we form $\wG_H$ from it by selecting $k - k'$ vertices in the non-neighborhood of $H$, with probability at least $\gamma / 40$ the maximum independent set of $\wG_H$ will have size exactly $k$, and any independent set of size $k$ can be formed by combining some independent set $I_H$ of $H$ with the selected set $I'$ in the non-neighborhood of $H$.
Therefore, given $\wG_H$ as input, algorithm $\Aa$ finds the independent set $I = I_H \cup I'$ of size $k$, which is the maximum independent set in $\wG_H$, with probability of at least $\gamma^2/80$.
Since $I_H\subset I$ and we know from construction what vertices of $\wG_H$ are the vertices of $H$, given the maximum independent set $I$ of $\wG_H$ we immediately obtain the maximum independent set $I_H$ of $H$.
Therefore, if we run $\Aa$ on $O(\frac{80}{\gamma^2})$ random instances of graphs $\wG_H$ (which we can create efficiently), with high probability algorithm $\Aa$ will give us some maximum independent set $I_H$ of $H$.
Meanwhile, by \cref{nph}, there exist instances of graphs $H$ where finding maximum independent set is NP-hard.
This finishes the proof of \cref{hardness}.

%{\em Remark.}
%We can also consider finding a maximum independent set of a graph $H$ of size $\polylog(n)$, with $p = 1/\polylog(n)$, 


==> smallp.tex <==
\section{Small values of $p$}\label{sec:constantClique}

In this section, we present a complete proof of \cref{thres2}.
\begin{theorem}[\cref{thres2} restated]\label{cllist}
	Let $p = o(n^{-2/T})$ for some integer $T > 1$.
	Let $G\sim AG(n, p, k)$, where $k \geq T$ is arbitrary.
	There is an (explicitly described) algorithm running in  time $O(n^{\frac{T}{4} + \frac{9}{2}})$ that almost surely for every possible adversarial choice of $k$ vertices finds the maximum clique of $G$.
\end{theorem}
The proof relies heavily on the following lemma.
\begin{lemma}\label{count}
	For every $k$, the number of maximal cliques in $G \sim AG(n, p, k)$ is at most the total number of the cliques in the original random graph $G(n, p)$.
\end{lemma}
\begin{proof}
	Let $G = (V, E)$ and let $K\subseteq V$ be the planted clique.
	We will count the maximal cliques in $G$, take an arbitrary clique $Q\subseteq V$.
	
	Suppose that $Q \subseteq V\setminus K$.
	If $Q$ is a maximal clique in $G[V\setminus K]$, then it is either maximal in $G$, or we can add some vertices from $K$ to form a maximal clique in $G$. 
	Observe that there is a unique way of adding vertices from $K$ to $Q$ to form a maximal clique (since $K$ is a clique itself).
	As a result, the maximal clique $Q$ in $G[V\setminus K]$ corresponds to exactly one maximal clique in $G$, and by counting $Q$ we count exactly one maximal clique in $G$.
	On the other hand, if $Q$ is not maximal in $G[V\setminus K]$ then it does not produce any additional cliques in $G$.
	Indeed, if we add some vertices from $V\setminus K$, we will either get a maximal clique in $G[V\setminus K]$, which is already counted, or another non-maximal clique.
	Suppose that we are adding some vertices from $K$.
	Note that if we get a maximal clique after adding vertices from $K$, we should have added the common neighborhood of $Q$ in $K$, and there is no other common neighbor of $Q$ in $V\setminus K$ which has the same neighborhood in $K$.
	Hence, this set $Q$ corresponds to at most one unique maximal clique in $G$.
	
	Suppose that $Q\subseteq K$.
	To create a maximal clique, we can try adding some vertices from $K$ or from $V\setminus K$.
	If we add vertices from $V\setminus K$, it would be equivalent to taking a subset from $V\setminus K$ that forms a maximal clique in $G[V\setminus K]$, which is already counted.
	On the other hand, if we add vertices only from $K$, then we should add all vertices from $K$, since $K$ is a clique.
	In any case, every set $Q\subseteq K$ that was a clique in the original graph corresponds to at most one not counted clique in $G$.
	
	Tu sum up, every clique in the original graph corresponds to at most one maximal clique in $G$.
	Then, the number of maximal cliques in $G$ is at most the number of cliques in the original random graph. 
\end{proof}
\begin{proof}[Proof of \cref{cllist}]
    Observe first that $p = n^{-2/T}$ is a threshold probability for cliques of size $T + 1$ in $G(n, p)$.
    Therefore, when $p = o(n^{-2/T})$, almost surely there are no cliques of size greater than $T$ in $G(n, p)$.
    Let's estimate the number of cliques of size at most $T$ in $G(n, p)$.
    Let $1 \leq t \leq T$, and let $X_t$ be the number of cliques of size $t$.
    It is clear that $X_t = \Bin\big(\binom{n}{t}, p^{\binom{t}{2}}\big)$, and by Chernoff bound, almost surely $X_t \leq (1 + o(1))\binom{n}{t}p^{\binom{t}{2}}$.
    Hence, the total number of cliques of size at most $T$ in $G(n, p)$ is
    \begin{multline*}
    \sum_{t = 3}^TX_t \leq (1 + o(1))\sum_{t = 3}^T\binom{n}{t}p^{\binom{t}{2}} 
    \leq \\\leq(1/T + o(1))\sum_{t = 3}^T\exp\left(\log np - \frac{t - 3}{t - 1}\log n\right)^{\frac{t(t - 1)}{2}} \leq \\\leq
    (1/T + o(1))\sum_{t = 3}^T\exp\left(\left(\frac{T- 2}{T} - \frac{t - 3}{t - 1}\right)\log n\right)^{\frac{t(t - 1)}{2}}.
    \end{multline*}
    It is easy to see that the summands increase as long as $t < T/2$, and then they start to decrease, so
    %Indeed,
    %\begin{gather*}
    %\frac{t(t - 1)}{2}\left(\frac{T- 2}{T} - \frac{t - 3}{t - 1}\right) < \frac{t(t + 1)}{2}\left(\frac{T- 2}{T} - \frac{t - 2}{t}\right) \iff\\
    %\iff (t - 1)\frac{T - 2}{T} - t + 3 < (t + 1)\frac{T - 2}{T} - \frac{(t + 1)(t - 2)}{t} \iff \\
    %\iff 2 < 2\left(\frac{T - 2}{T} + \frac{1}{t}\right) \iff 1 < \frac{T - 2}{T}  + \frac{1}{t} \iff \frac{2}{T} < \frac{1}{t} \iff t < \frac{T}{2}.
    %\end{gather*}
    the maximum summand is the one with $t = T/2$, which is equal to
    \begin{multline*}
    \exp\left(\left(\frac{T- 2}{T} - \frac{T/2 - 3}{T/2 - 1}\right)\log n\right)^{\frac{T(T/2 - 1)}{4}} =\\
    = \exp\left(\left(\frac{T - 2}{T} - \frac{T - 6}{T - 2}\right)\frac{T(T - 2)}{8}\log n\right) = n^{\frac{T}{4} + \frac{1}{2}},
    \end{multline*}
    and with high probability
    \[\sum_{t = 3}^TX_t \leq (1/T + o(1))\sum_{t = 3}^T\exp\left(\left(\frac{T- 2}{T} - \frac{t - 3}{t - 1}\right)\log n\right)^{\frac{t(t - 1)}{2}} \leq (1 + o(1))n^{\frac{T}{4} + \frac{1}{2}}.\]

	By \cref{count} and the observation above, almost surely there are at most $(1 + o(1))n^{\frac{T}{4} + \frac{1}{2}}$ maximal cliques in $G$.
	To list all maximal cliques in $G$, we can use, for example, the algorithm by K. Makino and T. Uno \cite{MU04}, with running time $O(\dmax(G)^4\mu(G))$ where $\mu(G)$ is the number of maximum cliques in $G$ and $\dmax(G)$ is the maximum degree of $G$.
	Since $\dmax(G) \leq n$ and $\mu(G)\leq  (1 + o(1))n^{\frac{T}{4} + \frac{1}{2}}$, we obtain a polynomial running time of $O(n^{\frac{T}{4} + \frac{9}{2}})$.
\end{proof}

%Let $p = p(n) = w(n)/n$ for some function $w(n)$.
%Observe that, for any integer  $T > 1$, if $w(n) = o(n^{1 - 2/T})$ then the size of the maximum clique in $G(n, p)$ is at most $T$ with high probability.
%Indeed, let $X$ be the number of cliques of size $T + 1$ in $G(n, p)$, then
%\begin{multline*}
%\P{X \geq 1} \leq \E{X} = \binom{n}{T + 1}p^{\binom{T + 1}{2}} \leq n^{T + 1}\cdot \frac{w(n)^{\frac{T(T + 1)}{2}}}{n^{\frac{T(T + 1)}{2}}} = \\=n^{T + 1- \frac{T(T + 1)}{2}}\cdot o\left(n^{\frac{T(T + 1)}{2} - T - 1}\right) = o(1),
%\end{multline*}
%so with probability tending to 1 there are no cliques of size greater than $T$ in $G(n, p)$.
%Actually, $p = p(n) = n^{-2/T}$ is a threshold probability for cliques of size $T + 1$ in $G(n, p)$.

%Let $w(n) = o(n^{1 - 2/T})$ for some integer $T$, % and $w(n) = \Om{n^{1 - 2/(T - 1)}}$ 
%so $T$ is the maximum possible size of the clique.

%The following theorem shows that if $p$ is small enough, we can find the maximum clique of $G\sim AG(n, p, k)$ for any value of parameter $k$.
%\begin{theorem}\label{cllist}
%	Let $p = p(n) = w(n)/n$ for $w(n) = o(n^{1 - 2/T})$ for integer $T > 1$.
%	Let $G\sim AG(n, p, k)$, where $k = k(n) \geq T$ is arbitrary.
%	There exists a polynomial time algorithm that with high probability fir every possible choice of $k$ vertices by the adversary finds the maximum clique of $G$.
%\end{theorem}


